Controlling infectious diseases: the decisive phase effect on a seasonal vaccination strategy

The study of epidemiological systems has generated deep interest in exploring the dynamical complexity of common infectious diseases driven by seasonally varying contact rates. Mathematical modeling and field observations have shown that, under seasonal variation, the incidence rates of some endemic infectious diseases fluctuate dramatically and the dynamics is often characterized by chaotic oscillations in the absence of specific vaccination programs. In fact, the existence of chaotic behavior has been precisely stated in the literature as a noticeable feature in the dynamics of the classical Susceptible-Infected-Recovered (SIR) seasonally forced epidemic model. However, in the context of epidemiology, chaos is often regarded as an undesirable phenomenon associated with the unpredictability of infectious diseases. As a consequence, the problem of converting chaotic motions into regular motions becomes particularly relevant. In this article, we consider the phase control technique applied to the seasonally forced SIR epidemic model to suppress chaos. Interestingly, this method of controlling chaos takes on a clear meaning as a weak perturbation on a seasonal vaccination strategy. Numerical simulations show that the phase difference between the two periodic forces - contact rate and vaccination - plays a very important role in controlling chaos.

==> apalike.tex <==
%% @texfile{
%%   author = "Oren Patashnik",
%%   version = "0.99b",
%%   date = "29 Feb 1992",
%%   filename = "apalike.tex",
%%   address = "Please use electronic mail",
%%   checksum = "103     854    5370",
%%   email = "opbibtex@cs.stanford.edu",
%%   codetable = "ISO/ASCII",
%%   supported = "yes",
%%   docstring = "Defines macros that make apalike work with plain TeX",
%% }
% apalike.tex, version 0.99b, for btxmac 0.99i, BibTeX 0.99c, TeX 3.0 or later.
% Copyright (C) 1990--92; all rights reserved.
% You may copy this file provided: that it's accompanied by btxmac.tex;
% and that either you make absolutely no changes to your copy, or if you
% do make changes, (1) you name the file something other than
% `apalike.tex' and you remove all occurrences of `apalike.tex' from the
% file, (2) you put, somewhere in the first twenty lines of the file,
% your name, along with an electronic address at which others who might
% use the file may reach you, and (3) you remove each occurrence of
% Oren's name and electronic address from this file.  These restrictions
% help ensure that all standard versions of these macros are identical,
% and that Oren doesn't get deluged with inappropriate e-mail.
%
% This file, apalike.tex, contains TeX macros that let you use the
% apalike bibliography style with plain TeX.  In essence, this file
% provides the TeX counterpart to apalike.sty, the LaTeX style file
% required for using the apalike bibliography style.  Please report any
% bugs (outright goofs, misfeatures, or unclear documentation) to Oren
% Patashnik (opbibtex@cs.stanford.edu).  These macros will become frozen
% shortly after BibTeX version 1.00 is released.
%
% AMS-TEX WARNING: This style (apalike) doesn't work with AmS-TeX's
% `amsppt' style, because AmS-TeX redefines the tie character `~' of
% plain TeX, and the `amsppt' style redefines plain TeX's `\nobreak'
% macro, so that a multiple-author reference for which `apalike'
% automatically produces an in-text citation like `(Jones et~al., 1992)'
% will throw AmS-TeX's `amsppt' style into an infinite loop, exceeding
% its input stack size.  (I've checked no other AmS-TeX styles for this
% problem.)  The AmS-TeX warning of btxmac.tex gives more information.
% END OF AMS-TEX WARNING.
%
% Editorial note (i.e., flame):
% Many journals require a style like `apalike', but I recommend that you
% not use it if you have a choice---use something like `plain' instead.
% Mary-Claire van Leunen (A Handbook for Scholars, Knopf, 1979) argues
% convincingly that a style like `plain' encourages better writing than
% one like `apalike'.  Furthermore the best argument for using an
% author-date style like `apalike'---that it's "the most practical"
% (The Chicago Manual of Style, University of Chicago Press, thirteenth
% edition, 1982, pages 400--401)---falls flat on its face with the new
% computer-typesetting technology.  For instance page 401 of the Chicago
% Manual anachronistically states "The chief disadvantage of [a style
% like `plain'] is that additions or deletions cannot be made after the
% manuscript is typed without changing numbers in both text references
% and list."  With (La)TeX the disadvantage obviously evaporates.
% Moreover, apalike indulges in what I think is a shortsighted practice:
% automatically abbreviating first names.  Abbreviating may occasionally
% make the work a page shorter, but at the cost of a less useful
% reference list; that's too high a cost for such a marginal benefit.
% The offense isn't egregious for a name like `Donald E. Knuth'---at
% least among those familiar with his field---since there aren't many
% other `D. E. Knuth's floating around.  But referring to `D. E. Smith'
% in a field having more than one can be quite confusing.  Moreover,
% with the proliferation of computers and citation indexes nowadays,
% it's important to indicate in the reference list an author's name
% exactly as it appears in the work cited.  Automatically abbreviating
% first names is simply bad scholarship.  (End of flame.)
%
% To use these macros you need the btxmac.tex macros, which let you use
% BibTeX with plain TeX (rather than with LaTeX); the file btxmac.tex
% explains those macros in detail, and gives examples.  You simply
% \input apalike right after you \input btxmac to invoke these macros.
%
%
%   HISTORY
%
% Oren Patashnik wrote the original version of these macros in December
% 1990, for use with btxmac.tex.
%
%   12-Dec-90  Version 0.99a, first general release.
%   29-Feb-92  0.99b, changed `\biblabelextrahang' to `\biblabelextraspace',
%                     to keep up with btxmac.tex version 0.99i.
%
%
% Here, finally (I swear, I thought he was never gonna stop), are the
% macros.  The first bunch makes the label empty and sets 2em of
% hanging indentation (via \biblabelextraspace) for each entry.
%
\def\biblabelprint#1{\noindent}%
\def\biblabelcontents#1{}%
\def\bblhook{\biblabelextraspace = 2em }%
%
%
% And the last bunch formats an in-text citation: parens around the
% entire citation; semicolons separating individual references; and a
% comma between a reference and its note (like `page 41') if it exists.
%
\def\printcitestart{(}%         left paren
\def\printcitefinish{)}%        right parent
\def\printbetweencitations{; }% semicolon, space
\def\printcitenote#1{, #1}%     comma, space, note (if it exists)

